Improving Factual Consistency in Summarization with Compression-Based Post-Editing

State-of-the-art summarization models still struggle to be factually consistent with the input text. A model-agnostic way to address this problem is post-editing the generated summaries. However, existing approaches typically fail to remove entity errors if a suitable input entity replacement is not available or may insert erroneous content. In our work, we focus on removing extrinsic entity errors, or entities not in the source, to improve consistency while retaining the summary's essential information and form. We propose to use sentence-compression data to train the post-editing model to take a summary with extrinsic entity errors marked with special tokens and output a compressed, well-formed summary with those errors removed. We show that this model improves factual consistency while maintaining ROUGE, improving entity precision by up to 30% on XSum, and that this model can be applied on top of another post-editor, improving entity precision by up to a total of 38%. We perform an extensive comparison of post-editing approaches that demonstrate trade-offs between factual consistency, informativeness, and grammaticality, and we analyze settings where post-editors show the largest improvements.

==> tables/prev.tex <==
% \caption{Example illustrating post-editing approaches. Entity swap \cite{chen-etal-2021-improving} does not modify the summary if a suitable entity replacement is not found, revision-based editing \cite{adams2022redress} performs more extensive changes, deletion \cite{wan2022factpegasus} removes errors but affects grammaticality, while our approach compresses the summary.}
% example 249 in test set
%  1772
%  3482
% \multirow{4}{\linewidth}{Kevin Patrick Dawes, 33, was abducted in 2012 as he entered Syria. ... The Czech government, ..., helped secure his release.} & Original & A US contractor who was held hostage in Syria \textcolor{red}{for more than three years} has been freed. \\
% & Entity Swap & -  \\
% & Rewrite & A US contractor who was held hostage in Syria has been freed \textit{by Czech authorities}. \\
% & Compress & A US contractor who was held hostage in Syria has been freed. \\ \hline
% \end{tabular}}
% \caption{Example illustrating varying approaches to post-editing. Entity swap \cite{chen-etal-2021-improving} fails to modify the summary as a suitable replacement is not present in the source, revision-based editing \cite{adams2022redress} performs more extensive changes, including entity insertion, while our sentence compression performs a single deletion operation. \af{wip - rewrite one looks v good here but can insert wrong entities}}

% \begin{table}[t!]
% \small
% \centering
%  \resizebox{\columnwidth}{!}{\begin{tabular}{|l | c c c | c c c|}
% \hline
% Model & E-P$_{src}$ & BS-P$_{src}$ & D$_{arc}$ &  BS-F1$_{ref}$ & R1 & R1-c \\ \hline
% UniLM & 60.63 & 42.45 & 0.83 & \textbf{46.07} & \textbf{42.13} & 40.74   \\ 
% \hspace{1mm} FASumFC &  60.66 & 42.40 & 0.83 & \textbf{46.00} &  \textbf{42.17}  & 40.78  \\ 
% \hspace{1mm} ReDRESS & 76.01 & \textbf{46.28} & 0.90 & 44.46 & 40.73 & 40.33   \\ 
% \hspace{1mm} FactPegasus &  \textbf{99.06} & 43.28 & 0.91 & 41.66 &  39.26   & \textbf{41.05}  \\ 
% \hspace{1mm} SentComp (ours) &  \textbf{80.72} & 43.86 & 0.89 & 44.45 &  40.79  & \textbf{40.93}  \\ 
% \hspace{1mm} ReDRESS + SentComp & 78.44 & \textbf{45.43} & 0.92 & 42.83  &  39.17  &   39.46  \\ \hline
% FASum & 71.01 & 37.17 & 0.71 & 33.32 &  30.27   &  29.90 \\ 
% \hspace{1mm} FASumFC & 68.59 & 37.03 & 0.71 & 33.23 &  30.19 & 29.83  \\ 
% \hspace{1mm} ReDRESS &  83.26 &  \textbf{44.56} & 0.88 & \textbf{35.97} & \textbf{32.76} & \textbf{32.91}  \\ 
% \hspace{1mm} FactPegasus &  \textbf{97.81} & 37.03 & 0.77 & 33.23 &  29.52  &  30.01  \\ 
% \hspace{1mm} SentComp (ours) & \textbf{89.32} & 37.99 & 0.77 & 33.73 &  30.54  & 30.63  \\ 
% \hspace{1mm} ReDRESS + SentComp &   83.04 & \textbf{43.17} &  0.89 &\textbf{36.01} &  \textbf{32.49} &  \textbf{32.88} \\ \hline
% BottomUp & 43.31 & 31.38 & 0.41 & 27.87 &  26.90  &  26.28  \\ 
% \hspace{1mm} FASumFC & 44.76 & 32.09 & 0.43 & 28.67 &  28.19  &  27.50  \\ 
% \hspace{1mm} ReDRESS &   82.11 & \textbf{45.70} & 0.85 & \textbf{34.21} & \textbf{31.50} & \textbf{31.62}  \\ 
% \hspace{1mm} FactPegasus &  \textbf{91.35} & 31.65 &  0.49 & 27.27 &  26.78  &  26.71 \\ 
% \hspace{1mm} SentComp (ours) & 79.74 & 34.13 &  0.54 & 30.06 &  27.65 &  28.40 \\ 
% \hspace{1mm} ReDRESS + SentComp &  \textbf{83.66}  & \textbf{44.30} & 0.87 & \textbf{34.38} &  \textbf{31.67} &  \textbf{32.03} \\ \hline
% TConvs2s & 70.58 & 36.93 & 0.72 & 33.77 &  31.45 &  31.00 \\ 
% \hspace{1mm} FASumFC & 69.53 & 36.57 & 0.73 & 34.21 &  32.43 &  31.95 \\ 
% \hspace{1mm} ReDRESS &  83.49 & \textbf{45.17} & 0.88 & \textbf{36.68} & \textbf{33.59} &  \textbf{33.71} \\ 
% \hspace{1mm} FactPegasus &  \textbf{97.56} & 37.44 & 0.77 &  32.61 & 30.57  & 31.08   \\ 
% \hspace{1mm} SentComp (ours) & \textbf{88.08} & 38.80 & 0.79 & 35.04 &  32.04 &  32.06  \\ 
% \hspace{1mm} ReDRESS + SentComp &  83.02  & \textbf{43.62} & 0.90 & \textbf{36.64} &  \textbf{33.17} &  \textbf{33.55} \\ \hline
% \end{tabular}}
% \caption{Comparison of best-performing post-editors with FASumFC \cite{zhu-etal-2021-enhancing} on UniLM \cite{unilm}, FASum \cite{zhu-etal-2021-enhancing}, BottomUp \cite{gehrmann-etal-2018-bottom}, TConvS2S \cite{pmlr-v70-gehring17a} outputs on XSum.
% } \label{table-fasum_result}
% \end{table}



% \af{May include others like \citet{cao-etal-2020-factual} if time permits for reference, although that barely corrects summaries.}
% 
% \noindent \textbf{SpanFact-QA} We implement the iterative QA post-editor from \citet{dong-etal-2020-multi}.  \af{Write that we do not include it.}
% 
% We train an Electra \cite{clark2020electra} QA model on to answer cloze-style questions by individually masking each of the entities in the reference summary as a separate question. 
% 
% During inference the entities in the summary are similarly masked and given to the QA model one-by-one.
% \begin{table*}[t!]
% \small
% \centering
% \resizebox{\linewidth}{!}{\begin{tabular}{| l | c c  c c  c | c c c c c c | c | c |}
% \hline
% Model & E-P$_{src}$ & BS-P$_{src}$ & D$_{arc}$ & QAFE & NLI & E-R$_{ref}$ & BS-F1$_{ref}$ & R1 & R2 & RL & R1-c & CoLA & Edit\% \\ \hline
% \multicolumn{13}{|c|}{XSUM} \\ \hline
% BART & 61.59 & 41.69 & 82.80 & 1.960 & 21.61 & 55.02 & 48.88 & 45.20 & 21.95 & 36.95 & 43.59 & 98.83 & - \\
% BART-c & 80.42 & 44.39 & 89.53 & 2.161 & 24.35 & 41.47 & 44.83 & 41.10 & 17.63 & 33.10 & 41.32 & 98.81 & - \\ \hline
% SpanFact \tiny \cite{dong-etal-2020-multi} & 61.96 & 41.70 & 82.90 & 1.947 & 21.59 & \textbf{54.51} & \textbf{48.77} & \textbf{45.10} & \textbf{21.88} & \textbf{36.88} & 43.54 & \textbf{98.77} & 40.53\\
% SpanFact-c & 74.26 & 42.82 & 85.85 & 1.978 & 21.15 & 45.20 & 47.32 & 43.44 & 19.80 & 35.42 & 43.45 & 98.44 & 60.27\\
% CCGS \tiny \cite{chen-etal-2021-improving} & 64.80 & 41.93 & 83.44 & 1.938 & 21.45 & \textbf{53.22} & \textbf{48.56} & \textbf{44.89} & \textbf{21.61} & \textbf{36.71} & 43.57 & 98.54 & 15.07 \\
% ReDRESS \tiny \cite{adams2022redress} & 75.42 & \textbf{44.90} & 88.54 & \textbf{2.168} & 23.26 & 47.37 & 46.98 & 43.30 & 20.12 & 35.29 & 42.81 & \textbf{98.79} & 61.82 \\
% FactPegasus \tiny \cite{wan2022factpegasus} & \textbf{98.71} & 42.82 & \textbf{90.82} & 2.082 & 23.56 & 35.76 & 44.39 & 41.98 & 18.30 & 34.45 & \textbf{43.98} & 93.25 & \textbf{67.05} \\
% SentCompFact-c (ours) & 80.02 & 43.03 & 88.35 & 2.124 & \textbf{23.77} & 44.49 & 47.00 & 43.45 & 20.29 & 35.63 & \textbf{43.61} & 98.61 & 54.31 \\
% ReDRESS + SentCompFact-c & \textbf{85.07} & \textbf{45.39} & \textbf{90.61} & \textbf{2.224} & \textbf{24.23} & 42.20 & 45.97 & 42.32 & 19.19 & 34.53 & 42.67 & 98.66 & \textbf{73.36} \\ \hline
% \multicolumn{13}{|c|}{CNN/DM} \\
% \hline
% BART & 98.50 & 71.10 & 98.57 & 4.550 & 84.79 & 58.93 & 43.55 & 44.05 & 21.12 & 41.02 & 44.11 & 95.68 & -  \\
% BART-c & 97.60 & 68.59 & 97.88 & 4.405 & 78.31 & 58.00 & 43.70 & 44.09 & 20.89 & 41.11 & 44.14 & 95.11 & -  \\ \hline
% SpanFact \tiny \cite{dong-etal-2020-multi} & 98.46 & 71.06 & 98.49 & 4.545 & 84.88 & 58.32 & 43.45 & 43.97 & 21.02 & 40.95 & 44.03 & \textbf{95.60} & 28.29 \\
% SpanFact-c & 98.83 & 71.07 & 98.53 & 4.544 & 85.02 & 58.19 & 43.41 & 43.95 & 20.99 & 40.93 & 44.01 & 95.50 & 32.36 \\
% CCGS \tiny \cite{chen-etal-2021-improving} & 98.18 & 71.04 & 98.49 & 4.466 & 83.41 & 58.00 & 43.48 & \textbf{43.98} & 21.03 & \textbf{40.96} & 44.04 & 95.48 & 14.93 \\
% ReDRESS \tiny \cite{adams2022redress} & 99.03 & \textbf{71.32} & 98.66 & \textbf{4.557} & \textbf{85.19} & \textbf{58.81} & \textbf{43.53} & \textbf{43.98} & \textbf{21.08} & \textbf{40.96} & 44.05 & \textbf{95.66} & \textbf{30.13} \\
% FactPegasus \tiny \cite{wan2022factpegasus} & \textbf{99.94} & 71.10 & 98.68 & 4.543 & 85.11 & 58.40 & 43.44 & \textbf{43.98} & 21.03 & \textbf{40.96} & \textbf{44.12} & 95.21 & 13.44 \\
% SentCompFact-c (ours) & \textbf{99.10} & 71.13 & \textbf{98.75} & 4.554 & \textbf{85.40} & \textbf{58.61} & \textbf{43.50} & \textbf{44.02} & \textbf{21.08} & \textbf{41.01} & \textbf{44.11} & 95.52 & 27.93 \\
% ReDRESS + SentCompFact-c & 98.95 & \textbf{71.24} & \textbf{98.74} & \textbf{4.555} & 83.64 & 58.49 & 43.44 & 43.96 & 21.04 & 40.95 & 44.04 & 95.42  & \textbf{44.53} \\ \hline
% \end{tabular}}
% \caption{Baseline and post-editing automatic results for factual consistency, relevance, and grammaticality metrics. The top two scores from the post-editors in each column are highlighted. 
% } \label{table-main-result}
% \end{table*}

% \begin{table}[t!]
% \small
% \centering
%  \resizebox{\columnwidth}{!}{\begin{tabular}{|l|c|ccc|c|}
% \hline
% Model & E-P$_{src}$ & R-1 & R-2 & R-L & CoLA \\ \hline
% UniLM & 60.63 & 42.13 & 19.53 & 34.16 & 97.33  \\ 
% \hspace{3mm} FASumFC &  60.66 & 42.17 & 19.54 & 34.19 & 97.00 \\ 
% \hspace{3mm} ReDRESS &  & & & & \\
% \hspace{3mm} FactPegasus &  99.06 & 39.24 & 16.19 & 31.86 &  92.30  \\ 
% \hspace{3mm} SentCompFact (ours) &  80.72 & 40.78 & 18.09 & 33.14 & 96.18  \\
% \hspace{3mm} ReDRESS + SentCompFact &  & & & & \\  \hline
% FASum & 71.01 & 30.27 & 10.02 & 23.80 & 92.99   \\ 
% \hspace{3mm} FASumFC & 68.59 & 30.19 & 9.96 & 23.72 & 93.39  \\ 
% \hspace{3mm} ReDRESS &  & & & & \\
% \hspace{3mm} FactPegasus &  97.81 & 29.52 & 9.19  & 23.72  & 89.28 \\ 
% \hspace{3mm} SentCompFact (ours) & 89.32 & 30.54 &  10.07 & 24.05 & 93.48  \\ 
% \hspace{3mm} ReDRESS + SentCompFact &  & & & & \\  \hline
% TConvs2s & 70.58 & 31.45 & 11.37 & 25.50 & 90.41 \\ 
% \hspace{3mm} FASumFC & 69.53 & 32.43 & 11.83 & 26.06 & 90.78 \\ 
% \hspace{3mm} ReDRESS &  & & & & \\
% \hspace{3mm} FactPegasus &  97.56 & 30.57 & 10.40 & 24.84  & 86.81  \\ 
% \hspace{3mm} SentCompFact (ours) & 88.08 & 32.04 & 11.49 & 25.73 & 91.20 \\ 
% \hspace{3mm} ReDRESS + SentCompFact &  & & & & \\  \hline
% BottomUp & 43.31 & 26.90 & 7.66 & 19.99 & 63.14 \\ 
% \hspace{3mm} FASumFC & 44.76 & 28.19 & 8.00 & 20.70 & 62.83  \\ 
% \hspace{3mm} ReDRESS &  & & & & \\
% \hspace{3mm} FactPegasus &  91.35 & 26.78 & 7.30 & 19.97  & 56.83  \\ 
% \hspace{3mm} SentCompFact (ours) & 79.74 & 27.65 & 8.09 & 21.30 & 65.13 \\ 
% \hspace{3mm} ReDRESS + SentCompFact &  & & & & \\  \hline
% \end{tabular}}
% \caption{Results on the examples provided by \cite{zhu-etal-2021-enhancing}.
% } \label{table-fasum_result}
% \end{table}




% \begin{table*}[t!]
% \small
% \centering
% \begin{tabular}{| l | c c | c | c |c c c|}
% \hline
% %  & ColA
% Model & E-P$_{src}$ & E-R$_{ref}$ & QAFactEval & NLI & R1 & R2 & RL \\ \hline
% \multicolumn{8}{|c|}{XSUM} \\ \hline
% BART &  61.59 & 55.02  &  &  &  45.20 &	21.95 &	36.95  \\ \hline
% BART-c &  80.42 & 41.47 &  &  &	41.10 & 17.63 &	33.10 \\ \hline \hline
% SpanFact-QA & 61.96 & 48.18  &  &  & 43.70 &	20.54 &	35.79 \\ \hline
% SpanFact-AutoReg &  61.96 & \textbf{54.51}  &  &  & 45.10 &	21.88 &	36.88 \\ \hline
% SpanFact-AutoReg-c &  74.26 & 45.20  &  &  & 43.44 &	19.80 &	35.42 \\ \hline
% CCGS  &  64.80 & \textbf{53.22} &  &  & 44.89 & 21.61 & 36.71 \\ \hline
% ReDRESS & 75.46 & 47.31  &  &  &  43.27 &	20.12 &	35.27 \\ \hline
% FactPegasus &  \textbf{98.71} & 35.76  &  &  & 41.98 &	18.30 &	34.45 \\  \hline  
% AutoReg-comp (ours) &  \textbf{80.02} & 44.49  &  &  &  43.45 &	20.29 &	35.63 \\  \hline \hline
% \multicolumn{8}{|c|}{CNN/DM} \\
% \hline
% BART &  98.50 & 58.93  &  &  &  44.05 &	21.12 &	41.02 \\ \hline
% BART-c  &  97.60 & 58.00  &  &  &  44.09  &	20.89 &	41.11 \\ \hline \hline
% SpanFact-QA  &  &  &  &  &  \\ \hline
% SpanFact-AutoReg  &  98.46 & 58.32  &  &  & 43.97 & 21.02 & 40.95 \\ \hline
% SpanFact-AutoReg-c  &  98.83 & 58.19  &  &  & 43.95 & 20.99 & 40.93 \\ \hline
% CCGS   &  98.18 &  58.00 &  &  & 43.98 & 21.03 & 40.96 \\ \hline
% ReDRESS  & 99.03 & \textbf{58.81} &  &  & 43.98 & 21.08 & 40.96  \\ \hline
% FactPegasus  &  \textbf{99.94} & 58.40  &  &  & 43.98 & 21.03 & 40.96 \\  \hline 
% AutoReg-comp (ours)  &  \textbf{99.10} & \tetxbf{58.61}  &  &  &  44.02 & 21.08 & 41.01 \\  \hline
% \end{tabular}
% \caption{Post-editing automatic results of baselines and post-editors for factual consistency and informativeness metrics. In all cases a higher score is better, and the top two scores from the post-editors in each column are highlighted.
% } \label{table-main-result}
% \end{table*}





% \begin{table*}[t!]
% \small
% \centering
% \resizebox{\linewidth}{!}{\begin{tabular}{| l | c c | c c | c | c | c |c c c| c | c | }
% \hline
% %  & ColA
% Model & E-P$_{src}$ & E-R$_{ref}$ & BS-P$_{src}$ & BS-F1$_{ref}$ & D$_{arc}$ &  QAFE & NLI & R1 & R2 & RL & CoLA & R1-c \\ \hline
% \multicolumn{13}{|c|}{XSUM} \\ \hline
% BART &  61.59 & 55.02  & 41.69 & 48.88 &  82.80 & 1.960 & 21.61 &  45.20 &	21.95 &	36.95 & 98.83 & 43.59 \\ 
% BART-c &  80.42 & 41.47 &  44.39 & 44.83 & 89.53 &  2.161 & 24.35  & 41.10 & 17.63 &	33.10 & 98.81 & 41.32 \\  \hline
% SpanFact &  61.96 & \textbf{54.51}  & 41.70 & \textbf{48.77} & 82.90 & 1.947 & 21.59 & \textbf{45.10} &	\textbf{21.88} &	\textbf{36.88}  & \textbf{98.77} & 43.54 \\ 
% SpanFact-c &  74.26 & 45.20  & 42.82 & 47.32 & 85.85 &  1.978 & 21.15 & 43.44 &	19.80 &	35.42 & 98.44 & 43.45 \\ 
% CCGS  &  64.80 & \textbf{53.22} &  41.93 & \textbf{48.56} & 83.44 & 1.938 & 21.45  & \textbf{44.89} & \textbf{21.61} & \textbf{36.71} & 98.54 & 43.57 \\ 
% ReDRESS & 75.42 & 47.37  &  \textbf{44.90} & 46.98 & 88.54 & \textbf{2.168} & 23.26  &  43.30 & 20.12 & 35.29 & \textbf{98.79} & 42.81 \\ 
% FactPegasus &  \textbf{98.71} & 35.76  & 42.82 & 44.39 & \textbf{90.82} &  2.082 & 23.56  & 41.98 &	18.30 &	34.45 & 93.25  & 43.98 \\  
% SentCompFact-c (ours) & 80.02 & 44.49  &  43.03 & 47.00 & 88.35 & 2.124 & \textbf{23.77} &  43.45 &	20.29 &	35.63  & 98.61 & 43.61 \\  
% ReDRESS + SentCompFact-c & \textbf{85.07} & 42.20  & \textbf{45.39} & 45.97 & \textbf{90.61} & \textbf{2.224} & \textbf{24.23} & 42.32 & 19.19 &	34.53 & 98.66 & 42.67 \\   \hline
% \multicolumn{13}{|c|}{CNN/DM} \\
% \hline
% BART &  98.50 & 58.93  &  71.10 & 43.55 & 98.57 & 4.550 & 84.79 &  44.05 &	21.12 &	41.02   & \textbf{95.68} & 44.11 \\ 
% BART-c  &  97.60 & 58.00  &  68.59 & 43.70 & 97.88 & 4.405 & 78.31 &  44.09  &	20.89 &	41.11  & 95.11 & 44.14 \\  \hline
% SpanFact  &  98.46 & 58.32  & 71.06 & 43.45 & 98.49 &  4.545 & 84.88  & 43.97 & 21.02 & 40.95  & 95.60 & 44.03 \\ 
% SpanFact-c  &  98.83 & 58.19  &  71.07 & 43.41 & 98.53 & 4.544 & 85.02  & 43.95 & 20.99 & 40.93  & 95.50 & 44.01 \\ 
% CCGS   &  98.18 &  58.00 &  71.04 & 43.48 & 98.49 & 4.466 & 83.41  & \textbf{43.98} & 21.03 & \textbf{40.96} & 95.48 & 44.04 \\ 
% ReDRESS  & 99.03 & \textbf{58.81} &  \textbf{71.32} & \textbf{43.53} & 98.66 & \textbf{4.557} & \textbf{85.19} & \textbf{43.98} & \textbf{21.08} & \textbf{40.96} & \textbf{95.66} & 44.05 \\
% FactPegasus  &  \textbf{99.94} & 58.40  & 71.10 & 43.44 & 98.68 &  4.543 & 85.11  & \textbf{43.98} & 21.03 & \textbf{40.96} & 95.21 & \textbf{44.12} \\  
% SentCompFact-c (ours)  &  \textbf{99.10} & \textbf{58.61}  & 71.13 & \textbf{43.50} & \textbf{98.75} & 4.554 & \textbf{85.40}  &  \textbf{44.02} & \textbf{21.08} & \textbf{41.01} & 95.52 & \textbf{44.11} \\  
% ReDRESS + SentCompFact-c & 98.95 & 58.49  & \textbf{71.24} & 43.44  &  \textbf{98.74} & \textbf{4.555} & 83.64 & 43.96 & 21.04 & 40.95 & 95.42 & 44.04 \\   \hline
% \end{tabular}}
% \caption{Post-editing automatic results of baselines and post-editors for factual consistency and informativeness metrics. In all cases a higher score is better, and the top two scores from the post-editors in each column are highlighted.
% } \label{table-main-result}
% \end{table*}
% SpanFact-QA & 61.96 & 48.18  & 1.869 & 21.49  & 43.70 &	20.54 &	35.79 \\ 
% ReDRESS_prev & 75.46 & 47.31  &  2.167 & 23.26  &  43.27 &	20.12 &	35.27 \\ 
% SpanFact-QA  & 98.50 &  58.93 &  &  &  \\ 
% \resizebox{\columnwidth}{!}{}
% CCGS + SentCompFact-c (ours) & \textbf{81.70}  & 43.86 &  2.085 & 23.46  & 43.27 & 20.09	 &	 35.48 \\   \hline
% CCGS + SentCompFact-c (ours) &  99.13 &  58.38 &  4.51 &  84.78 &  43.99 & 20.03 & 40.97 \\  \hline






% \begin{table*}[t!]
% \small
% \centering
% \begin{tabular}{| l | c c | c c | c | c | c |c c c|}
% \hline
% %  & ColA
% Model & E-P$_{src}$ & E-R$_{ref}$ & BS-P$_{src}$ & BS-F1$_{ref}$ & D$_{arc}$ &  QAFactEval & NLI & R1 & R2 & RL \\ \hline
% \multicolumn{8}{|c|}{XSUM} \\ \hline
% BART &  61.59 & 55.02  & 41.69 & 48.88 &  82.80 & 1.960 & 21.61 &  45.20 &	21.95 &	36.95  \\ 
% BART-c &  80.42 & 41.47 &  2.161 & 24.35  &	41.10 & 17.63 &	33.10 \\  \hline
% % SpanFact-QA & 61.96 & 48.18  & 1.869 & 21.49  & 43.70 &	20.54 &	35.79 \\ 
% SpanFact &  61.96 & \textbf{54.51}  &  1.947 & 21.59 & 45.10 &	21.88 &	36.88 \\ 
% SpanFact-c &  74.26 & 45.20  &  1.978 & 21.15 & 43.44 &	19.80 &	35.42 \\ 
% CCGS  &  64.80 & \textbf{53.22} &  1.938 & 21.45  & 44.89 & 21.61 & 36.71 \\ 
% % ReDRESS_prev & 75.46 & 47.31  &  2.167 & 23.26  &  43.27 &	20.12 &	35.27 \\ 
% ReDRESS & 75.42 & 47.37  &  2.168 & 23.26  &  43.30 & 20.12 & 35.29 \\ 
% FactPegasus &  \textbf{98.71} & 35.76  &  2.082 & 23.56  & 41.98 &	18.30 &	34.45 \\  
% SentCompFact-c (ours) & 80.02 & 44.49  &   2.124 & 23.77 &  43.45 &	20.29 &	35.63 \\   \hline
% % CCGS + SentCompFact-c (ours) & \textbf{81.70}  & 43.86 &  2.085 & 23.46  & 43.27 & 20.09	 &	 35.48 \\   \hline
% ReDRESS + SentCompFact-c & 85.07 & 42.20  &   &  & 42.32 & 19.19 &	34.53 \\   \hline
% \multicolumn{8}{|c|}{CNN/DM} \\
% \hline
% BART &  98.50 & 58.93  & 4.550 & 84.79 &  44.05 &	21.12 &	41.02 \\ 
% BART-c  &  97.60 & 58.00  &  4.405 & 78.31 &  44.09  &	20.89 &	41.11 \\  \hline
% % SpanFact-QA  & 98.50 &  58.93 &  &  &  \\ 
% SpanFact  &  98.46 & 58.32  &  4.545 & 84.88  & 43.97 & 21.02 & 40.95 \\ 
% SpanFact-c  &  98.83 & 58.19  &   4.544 & 85.02  & 43.95 & 20.99 & 40.93 \\ 
% CCGS   &  98.18 &  58.00 &   4.466 & 83.41  & 43.98 & 21.03 & 40.96 \\ 
% ReDRESS  & 99.03 & \textbf{58.81} &  4.557 & 85.19 & 43.98 & 21.08 & 40.96  \\
% FactPegasus  &  \textbf{99.94} & 58.40  &  4.543 & 85.11  & 43.98 & 21.03 & 40.96 \\  
% SentCompFact-c (ours)  &  \textbf{99.10} & \textbf{58.61}  &  4.554 & 85.40  &  44.02 & 21.08 & 41.01 \\  \hline
% % CCGS + SentCompFact-c (ours) &  99.13 &  58.38 &  4.51 &  84.78 &  43.99 & 20.03 & 40.97 \\  \hline
% ReDRESS + SentCompFact-c &  &   &   &  &  &  &  \\   \hline
% \end{tabular}
% \caption{Post-editing automatic results of baselines and post-editors for factual consistency and informativeness metrics. In all cases a higher score is better, and the top two scores from the post-editors in each column are highlighted.
% } \label{table-main-result}
% \end{table*}
% % \resizebox{\columnwidth}{!}{}






% % \begin{table}[t!]
% % \small
% % \centering
% %  \resizebox{\columnwidth}{!}{\begin{tabular}{|l|c|ccc|}
% % \hline
% % Model & E-P$_{src}$ & R-1 & R-2 & R-L \\ \hline
% % UniLM & 60.63 & 42.13 & 19.53 & 34.16  \\ 
% % \hspace{3mm} FASumFC &  60.66 & 42.17 & 19.54 & 34.19 \\ 
% % \hspace{3mm} FactPegasus &  99.06 & 39.24 & 16.19 & 31.86  \\ 
% % \hspace{3mm} SentCompFact (ours) &  80.72 & 40.78 & 18.09 & 33.14  \\ \hline
% % FASum & 71.01 & 30.27 & 10.02 & 23.80 \\ 
% % \hspace{3mm} FASumFC & 68.59 & 30.19 & 9.96 & 23.72 \\ 
% % \hspace{3mm} FactPegasus &  97.81 & 29.52 & 9.19  & 23.72  \\ 
% % \hspace{3mm} SentCompFact (ours) & 89.32 & 30.54 &  10.07 & 24.05 \\ \hline
% % TConvs2s & 70.58 & 31.45 & 11.37 & 25.50 \\ 
% % \hspace{3mm} FASumFC & 69.53 & 32.43 & 11.83 & 26.06 \\ 
% % \hspace{3mm} FactPegasus &  97.56 & 30.57 & 10.40 & 24.84  \\ 
% % \hspace{3mm} SentCompFact (ours) & 88.08 & 32.04 & 11.49 & 25.73 \\ \hline
% % BottomUp & 43.31 & 26.90 & 7.66 & 19.99 \\ 
% % \hspace{3mm} FASumFC & 44.76 & 28.19 & 8.00 & 20.70 \\ 
% % \hspace{3mm} FactPegasus &  91.35 & 26.78 & 7.30 & 19.97  \\ 
% % \hspace{3mm} SentCompFact (ours) & 79.74 & 27.65 & 8.09 & 21.30 \\ \hline
% % \end{tabular}}
% % \caption{Results on the examples provided by \cite{zhu-etal-2021-enhancing}.
% % } \label{table-fasum_result}
% % \end{table}
% \begin{table}[t!]
% \small
% \centering
%  \resizebox{\columnwidth}{!}{\begin{tabular}{|l|c|ccc|c|}
% \hline
% Model & E-P$_{src}$ & R-1 & R-2 & R-L & CoLA \\ \hline
% UniLM & 60.63 & 42.13 & 19.53 & 34.16 & 97.33  \\ 
% \hspace{3mm} FASumFC &  60.66 & 42.17 & 19.54 & 34.19 & 97.00 \\ 
% \hspace{3mm} ReDRESS &  & & & & \\
% \hspace{3mm} FactPegasus &  99.06 & 39.24 & 16.19 & 31.86 &  92.30  \\ 
% \hspace{3mm} SentCompFact (ours) &  80.72 & 40.78 & 18.09 & 33.14 & 96.18  \\
% \hspace{3mm} ReDRESS + SentCompFact &  & & & & \\  \hline
% FASum & 71.01 & 30.27 & 10.02 & 23.80 & 92.99   \\ 
% \hspace{3mm} FASumFC & 68.59 & 30.19 & 9.96 & 23.72 & 93.39  \\ 
% \hspace{3mm} ReDRESS &  & & & & \\
% \hspace{3mm} FactPegasus &  97.81 & 29.52 & 9.19  & 23.72  & 89.28 \\ 
% \hspace{3mm} SentCompFact (ours) & 89.32 & 30.54 &  10.07 & 24.05 & 93.48  \\ 
% \hspace{3mm} ReDRESS + SentCompFact &  & & & & \\  \hline
% TConvs2s & 70.58 & 31.45 & 11.37 & 25.50 & 90.41 \\ 
% \hspace{3mm} FASumFC & 69.53 & 32.43 & 11.83 & 26.06 & 90.78 \\ 
% \hspace{3mm} ReDRESS &  & & & & \\
% \hspace{3mm} FactPegasus &  97.56 & 30.57 & 10.40 & 24.84  & 86.81  \\ 
% \hspace{3mm} SentCompFact (ours) & 88.08 & 32.04 & 11.49 & 25.73 & 91.20 \\ 
% \hspace{3mm} ReDRESS + SentCompFact &  & & & & \\  \hline
% BottomUp & 43.31 & 26.90 & 7.66 & 19.99 & 63.14 \\ 
% \hspace{3mm} FASumFC & 44.76 & 28.19 & 8.00 & 20.70 & 62.83  \\ 
% \hspace{3mm} ReDRESS &  & & & & \\
% \hspace{3mm} FactPegasus &  91.35 & 26.78 & 7.30 & 19.97  & 56.83  \\ 
% \hspace{3mm} SentCompFact (ours) & 79.74 & 27.65 & 8.09 & 21.30 & 65.13 \\ 
% \hspace{3mm} ReDRESS + SentCompFact &  & & & & \\  \hline
% \end{tabular}}
% \caption{Results on the examples provided by \cite{zhu-etal-2021-enhancing}.
% } \label{table-fasum_result}
% \end{table}

==> tables/summcomp_overview.tex <==
\begin{table}[t!]
\small
\centering
 \resizebox{\columnwidth}{!}{\begin{tabular}{p{0.20\columnwidth}|p{0.40\columnwidth}|p{0.40\columnwidth}}
\hline
Model & Input & Output  \\
\hline 
Perturber & It was the season in which Chelsea played by their own record book. || 18 | the Champions League &  It was the \textcolor{red}{18 th consecutive season} in which Chelsea played by their own record book \textcolor{red}{in the Champions League}.  \\ \hline
Post-Editor & SRC ||  It was the \#\# 18 \#\# th consecutive season in which Chelsea played by their own record book in \#\# the Champions League \#\#. & It was the season in which Chelsea played by their own record book. \\ \hline
\end{tabular}}
\caption{Overview of our compression-based approach. A perturber model is trained to produce an uncompressed sentence conditioned upon the compressed sentence and an appended list of entities. Our post editor takes the source document (SRC) and a summary with entities to remove surrounded by special tokens and learns to remove the erroneous words.}
\label{tab:summ_comp}
\end{table}
